CaKE: Circuit-aware Editing Enables Generalizable Knowledge Learners

Knowledge Editing (KE) enables the modification of outdated or incorrect information in large language models (LLMs). While existing KE methods can update isolated facts, they often fail to generalize these updates to multi-hop reasoning tasks that rely on the modified knowledge. Through an analysis of reasoning circuits -- the neural pathways LLMs use for knowledge-based inference, we find that current layer-localized KE approaches (e.g., MEMIT, WISE), which edit only single or a few model layers, inadequately integrate updated knowledge into these reasoning pathways. To address this limitation, we present CaKE (Circuit-aware Knowledge Editing), a novel method that enhances the effective integration of updated knowledge in LLMs. By only leveraging a few curated data samples guided by our circuit-based analysis, CaKE stimulates the model to develop appropriate reasoning circuits for newly incorporated knowledge. Experiments show that CaKE enables more accurate and consistent use of edited knowledge across related reasoning tasks, achieving an average improvement of 20% in multi-hop reasoning accuracy on the MQuAKE dataset while requiring less memory than existing KE methods. We release the code and data in https://github.com/zjunlp/CaKE.

==> Table/70b.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\textwidth}{!}{% Resize table to fit within the text width
\begin{tabular}{cc|cc|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Model}}  & \multicolumn{2}{c|}{\textbf{MQUAKE-CF}} & \multicolumn{2}{c|}{\textbf{MQUAKE-CF-v2}} & \multicolumn{2}{c}{\textbf{MQUAKE-T}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
&& \textbf{H-Acc.$\uparrow$} & \textbf{MAcc.$\uparrow$} & \textbf{H-Acc.$\uparrow$} & \textbf{MAcc.$\uparrow$} & \textbf{H-Acc.$\uparrow$} & \textbf{MAcc.$\uparrow$} \\
\midrule
Pre-edited & & 75.6 &  34.7  & 76.8 & 37.7  & 60.1 & 15.6\\
\midrule
LoRA & \multirow{3}{*}{\rotatebox{90}{{L-70B}}}  & \underline{93.1} & \underline{53.2} & \underline{90.5} & \underline{50.2} & \underline{90.1} & \underline{90.6} \\
MeLLo& & 8.0 & 6.4 & 8.6 & 9.9 & 11.6 & 32.9 \\
CaKE(ours) & & \textbf{93.5} & \textbf{65.4} &  \textbf{93.3} & \textbf{63.3} &\textbf{91.1} & \textbf{94.6} \\\bottomrule
\end{tabular}
}
\caption{Comparison of \ours with existing methods on MQuAKE for LLAMA3-70B-Instruct. The best results are highlighted in bold, while the second-best results are underlined. Due to the computational limitations, we just ran the LoRA and MeLLo in the 70B model.
Here, LoRA for the 70B model is added for all layers because the performance on a single layer is extremely low.}
\vspace{-8pt}
\label{tab:70b_comp}
\end{table*}



==> Table/patch_tab.tex <==
\begin{table}[t]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{ccc}
\toprule
Model & Entity Patch & Relation Patch  \\ \midrule
LLaMA3-8B-Ins. & 85.35 & 56.20  \\ 
Qwen2.5-7B-Ins. & 97.29 & 55.40  \\ \bottomrule
\end{tabular}
}
\caption{Activation Patching Success Rates (\%).}
\vspace{-10pt}
\label{tab:patch}
\end{table}

